Calibration and operation of SiPM-based cameras for gamma-ray astronomy in presence of high night-sky light

The next generation of Cherenkov telescope cameras feature Silicon Photo Multipliers (SiPM), which can guarantee excellent performance and allow for observation also under moonlight, increasing duty-cycle and therefore the physics reach. A 4 m-diameter Davies-Cotton prototype telescope with a 9-degree optical FoV and a 1296-pixel SiPM camera, has been designed to meet the requirements of the next generation of ground-based gamma-ray observatories at the highest energies. The large-scale production of the telescopes for array deployment has required the development of a fully automated calibration strategy which relies on a dedicated hardware, the Camera Test Setup (CTS). For each camera pixel, the CTS is equipped with two LEDs, one operated in pulsed mode to reproduce signal and one in continuous mode to reproduce night-sky background. In this contribution we will present the camera calibration strategy, from the laboratory measurement to the on-site monitoring with emphasis on the results obtained with the first camera prototype. In addition, key performances such as charge resolution, time resolution and trigger efficiencies and their degradation with increasing night-sky background level will be presented.

==> abstract.tex <==

The next generation of Cherenkov telescope cameras feature Silicon Photo Multipliers (SiPM), which can guarantee excellent performance and allow for observation also under moonlight, increasing duty-cycle and therefore the physics reach. A 4 m-diameter Davies-Cotton prototype telescope with a 9-degree optical FoV and a 1296-pixel SiPM camera, has been designed to meet the requirements of the next generation of ground-based gamma-ray observatories at the highest energies.\\

The large-scale production of the telescopes for array deployment has required the development of a fully automated calibration strategy which relies on a dedicated hardware, the Camera Test Setup (CTS). For each camera pixel, the CTS is equipped with two LEDs, one operated in pulsed mode to reproduce signal and one in continuous mode to reproduce night-sky background.\\

In this contribution we will present the camera calibration strategy, from the laboratory measurement to the on-site monitoring with emphasis on the results obtained with the first camera prototype. In addition, key performances such as charge resolution, time resolution and trigger efficiencies and their degradation with increasing night-sky background level will be presented.\\

